Rethinking Optimization with Differentiable Simulation from a Global Perspective

Differentiable simulation is a promising toolkit for fast gradient-based policy optimization and system identification. However, existing approaches to differentiable simulation have largely tackled scenarios where obtaining smooth gradients has been relatively easy, such as systems with mostly smooth dynamics. In this work, we study the challenges that differentiable simulation presents when it is not feasible to expect that a single descent reaches a global optimum, which is often a problem in contact-rich scenarios. We analyze the optimization landscapes of diverse scenarios that contain both rigid bodies and deformable objects. In dynamic environments with highly deformable objects and fluids, differentiable simulators produce rugged landscapes with nonetheless useful gradients in some parts of the space. We propose a method that combines Bayesian optimization with semi-local 'leaps' to obtain a global search method that can use gradients effectively, while also maintaining robust performance in regions with noisy gradients. We show that our approach outperforms several gradient-based and gradient-free baselines on an extensive set of experiments in simulation, and also validate the method using experiments with a real robot and deformables. Videos and supplementary materials are available at https://tinyurl.com/globdiff

==> macro.tex <==
\usepackage[utf8]{inputenc}
\usepackage{amsmath,amsfonts,bbm}
\makeatletter
\g@addto@macro\normalsize{%
  \setlength\abovedisplayskip{4pt}
  \setlength\belowdisplayskip{4pt}
  \setlength\abovedisplayshortskip{4pt}
  \setlength\belowdisplayshortskip{4pt}
}
\usepackage[ruled,linesnumbered,vlined]{algorithm2e}
\usepackage{algpseudocode}
\usepackage{graphicx}
\usepackage{wrapfig}
\usepackage{booktabs}
\usepackage{adjustbox}
\usepackage{float}
\usepackage{makecell}
\usepackage[font={small}]{caption}
\usepackage{mathtools}
\usepackage[usenames,dvipsnames]{xcolor}
\usepackage{natbib}
\usepackage{verbatim}
\usepackage{tikz}
\usepackage{enumitem}  % for tighter list spacing
\usepackage{cancel}
\usepackage[user,titleref]{zref}
\usepackage{cancel}
\usepackage{wrapfig}
\usepackage{booktabs}
\usepackage{makecell}
\usepackage[colorinlistoftodos,backgroundcolor=yellow,bordercolor=yellow,linecolor=yellow,textcolor=gray,textsize=scriptsize]{todonotes}
\usepackage{etoolbox}
% for arXiv version
\usepackage{chngcntr}  % for appendix figures
\usepackage[page,header]{appendix}
\usepackage{titletoc}
\usepackage{setspace}
\renewcommand{\baselinestretch}{1.08}

% gray comments in algorithm
\newcommand\mycommfont[1]{\textcolor{gray}{#1}}
\SetCommentSty{mycommfont}

% remove extra horizontal whitespace for algorithm
% https://tex.stackexchange.com/questions/520327/remove-horizontal-spacing-on-the-right-with-algorithm2e
\makeatletter
% Remove right hand margin in algorithm
\patchcmd{\@algocf@start}% <cmd>
  {-1.5em}% <search>
  {0pt}% <replace>
  {}{}% <success><failure>
\makeatother

\makeatletter
\newcommand\fs@nobottomruled{\def\@fs@cfont{\bfseries}\let\@fs@capt\floatc@ruled
  \def\@fs@pre{\hrule height.8pt depth0pt \kern2pt}%
  \def\@fs@post{}% Formerly \def\@fs@post{\kern2pt\hrule\relax}%
  \def\@fs@mid{\kern2pt\hrule\kern2pt}%
  \let\@fs@iftopcapt\iftrue}
\makeatother

\newcommand{\todob}[1]{{\color{brown} TODO: {#1}}}
\newcommand{\info}[1]{{\color{Sepia} Info: {#1}}}

% change comment symbol in algorithm2e
\SetKwComment{Comment}{$\triangleright$\ }{}

% colors
\definecolor{darkgreen}{RGB}{40, 150, 40}
\definecolor{gray}{RGB}{140, 140, 140}
\newcommand{\rulesep}{\color{gray}\unskip\ \vrule\ }
\newcommand{\pink}[1]{{\color{magenta}#1}}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\diag}{diag}
\DeclareMathOperator*{\krdim}{krdim}
\DeclareMathOperator*{\codim}{codim}
\DeclareMathOperator*{\depth}{depth}
\newcommand{\eq}[1]{\begin{align*}#1\end{align*}}
\newcommand{\bmat}[1]{\begin{bmatrix}#1\end{bmatrix}}
\newcommand{\pmat}[1]{\begin{pmatrix}#1\end{pmatrix}}

\newcommand{\zn}{{z^{(n)}}}
\newcommand{\xn}{{x^{(n)}}}
\newcommand{\yn}{{y^{(n)}}}
\newcommand{\br}{{\pmb{r}}}
\newcommand{\bs}{{\pmb{s}}}
\newcommand{\bv}{{\pmb{v}}}
\newcommand{\bw}{{\pmb{w}}}
\newcommand{\bx}{{\pmb{x}}}
\newcommand{\by}{{\pmb{y}}}
\newcommand{\bz}{{\pmb{z}}}
\newcommand{\bmu}{{\pmb{\mu}}}
\newcommand{\bphi}{{\pmb{\phi}}}
\newcommand{\btau}{{\pmb{\tau}}}
\newcommand{\bth}{{\pmb{\theta}}}
\newcommand{\bxi}{{\pmb{\xi}}}
\newcommand{\bSigma}{{\pmb{\Sigma}}}
\newcommand{\R}{{\mathbb{R}}}
\newcommand{\C}{{\mathbb{C}}}
\newcommand{\E}{{\mathbb{E}}}
\newcommand{\M}{{\mathcal{M}}}
\newcommand{\N}{{\mathcal{N}}}
\newcommand{\OO}{{\mathcal{O}}}
\newcommand{\V}{{\mathcal{V}}}
\newcommand{\mf}{{\mathfrak{f}}}
\newcommand{\rar}{\rightarrow}
\newcommand{\lar}{\leftarrow}
\newcommand{\tnxt}{t\text{+}1}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
